Ordered Topological Deep Learning: a Network Modeling Case Study

Computer networks are the foundation of modern digital infrastructure, facilitating global communication and data exchange. As demand for reliable high-bandwidth connectivity grows, advanced network modeling techniques become increasingly essential to optimize performance and predict network behavior. Traditional modeling methods, such as packet-level simulators and queueing theory, have notable limitations --either being computationally expensive or relying on restrictive assumptions that reduce accuracy. In this context, the deep learning-based RouteNet family of models has recently redefined network modeling by showing an unprecedented cost-performance trade-off. In this work, we revisit RouteNet's sophisticated design and uncover its hidden connection to Topological Deep Learning (TDL), an emerging field that models higher-order interactions beyond standard graph-based methods. We demonstrate that, although originally formulated as a heterogeneous Graph Neural Network, RouteNet serves as the first instantiation of a new form of TDL. More specifically, this paper presents OrdGCCN, a novel TDL framework that introduces the notion of ordered neighbors in arbitrary discrete topological spaces, and shows that RouteNet's architecture can be naturally described as an ordered topological neural network. To the best of our knowledge, this marks the first successful real-world application of state-of-the-art TDL principles --which we confirm through extensive testbed experiments--, laying the foundation for the next generation of ordered TDL-driven applications.

==> sections/08-conclusion.tex <==
To the best of our knowledge, this work studies the first state-of-the-art TDL application to a real-world setting, supported by extensive testbed experiments. By formulating RouteNet within the TDL paradigm using OrdGCCNs, we reveal a deeper theoretical structure underlying its success, positioning network modeling as a naturally higher-order application domain.

==> sections/OLD-networking.tex <==
%- Overview of network modeling.
%- Traditional network modeling techniques (packet-level simulators, queueing theory).
%- Recent advances in deep learning for network modeling.
%- Introduction to topological deep learning.

\subsection{Overview of Network Modeling}
Network modeling is a cornerstone of computer network research, design, and operations. It enables the simulation and analysis of network behavior, which is crucial for tasks such as protocol development, performance evaluation, and network optimization. By abstracting the network’s physical and logical components, models help researchers and engineers predict performance metrics like delay under different configurations and workloads. Over the years, network modeling has been applied in diverse areas, including traffic engineering, capacity planning, and Quality of Service (QoS) assurance.

\subsection{Traditional Approaches to Network Modeling}
Two widely adopted techniques for network modeling are packet-level simulators and analytical models based on Queuing Theory (QT).

\subsubsection{Packet-Level Simulators}
Packet-level simulators, such as ns-3 and OMNeT++, provide detailed modeling by simulating network behavior at the granularity of individual packets. These tools offer high accuracy and flexibility, allowing researchers to include various features such as routing algorithms, scheduling policies, and traffic patterns. However, their main limitation is computational cost. Simulation time typically grows linearly with the number of packets processed, making these tools impractical for large-scale networks or real-time applications. For instance, simulating a high-speed link (e.g., 10 Gbps) over a realistic traffic volume can take hours or even days.

Efforts to address this limitation have focused on parallelizing the simulation process to improve efficiency. For instance, DONS (Distributed Omnet++ Simulation) \textbf{CITE DONS} achieves up to 65x speedup over traditional sequential simulators by partitioning networks and processing them in parallel. Similarly, approaches like Deep Queue Net (DQN) leverage transformers and multi-GPU configurations to significantly accelerate computational times.

Figure \ref{fig:simulation_cost} illustrates simulation times for several link speeds commonly found in modern networks. The results show that even with advancements like DONS and DQN, packet-level simulators remain computationally expensive, particularly for high-speed links. 

\begin{figure}[!htbp] \centering \includegraphics[width=\columnwidth]{./figures/motivation_cost_v2.pdf} \caption{Simulation times for various link speeds in modern networks using OMNeT++, DONS, and DQN. Results demonstrate the significant computational cost of packet-level simulations, even with advanced techniques.} \label{fig:simulation_cost} 
\end{figure}

\subsubsection{Queuing Theory}
Queuing Theory (QT) has been a basis of network modeling for decades and remains one of the most widely used analytical techniques in the field. Its importance stems from its ability to provide a mathematical framework to model networks as a set of interconnected queues. Each queue represents a network component, such as a router or switch, handling data packets. 

QT’s dominance in network modeling lies in its simplicity and efficiency. Unlike packet-level simulators, which require extensive computation to simulate individual packets, QT uses mathematical models to derive performance metrics directly. For example, it assumes that traffic follows a Poisson arrival process and that queues behave according to Markovian principles. These assumptions make QT computationally fast and well-suited for large-scale networks or scenarios where quick predictions are required.

\begin{table}[!htbp]
\caption{Delay prediction using the QT baseline for different traffic models. The error is computed w.r.t. simulation results.}
\label{tab:traffic_model_qt_delay}
\centering
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
     & MAPE & MSE & MAE & R\textsuperscript{2} \\
     \midrule
Poisson & 12.6\% & 0.001 & 0.017 & 0.998 \\
Deterministic & 22.4\% & 0.715 & 0.321 & 0.611 \\
On-Off & 23.1\% & 0.784 & 0.363 & 0.613 \\
A. Exponentials & 21.1\% & 0.686 & 0.316 & 0.618 \\
M. Exponentials & 68.1\% & 1.10 & 0.798 & 0.145 \\
Mixed & 35.1\% & 0.721 & 0.430 & 0.560 \\
\bottomrule
\end{tabular}%
}
\end{table}


However, the strength of QT is also its main limitation. The simplifying assumptions that make it efficient often fail to capture the complexities of real-world network traffic. Studies have shown that modern network traffic exhibits properties like strong autocorrelation and heavy-tailed distributions, which deviate significantly from the idealized Poisson and Markovian models. This is evident in the results shown in Table \ref{tab:traffic_model_qt_delay}, where QT's performance in delay prediction varies significantly across different traffic models.

For example, when traffic adheres to the Poisson arrival process—a core assumption of QT—the model achieves excellent accuracy, with a Mean Absolute Percentage Error (MAPE) of 12.6\% and an $R^2$ value of 0.998, indicating a near-perfect fit. However, as traffic patterns become more complex, such as with On-Off or mixed traffic models, the prediction errors increase substantially, with MAPE values exceeding 35\% in some cases. Notably, for traffic with high variance, like the Modulated Exponentials model, QT struggles the most, with a MAPE of 68.1\% and an $R^2$ of only 0.145. These results highlight QT's inability to generalize to traffic patterns that deviate from its core assumptions.


\subsection{Recent Advances in Network Modeling}
The limitations of traditional approaches, such QT and packet-level simulators, have driven the exploration of data-driven techniques, particularly those leveraging advancements in Deep Learning (DL). Unlike QT, which relies on strong assumptions about traffic characteristics, or packet-level simulators, which suffer from high computational overhead, DL-based models learn directly from real-world data. This enables these models to accurately represent the complex, non-linear relationships inherent in modern networks without the need for restrictive assumptions about traffic distributions or configurations.

%One of the key advantages of data-driven methods is their ability to generalize across a wide range of network scenarios. For instance, by training on diverse datasets, DL models can adapt to unseen topologies, routing schemes, and traffic patterns, which is a significant limitation of traditional methods. Furthermore, they are capable of extracting deep insights from data, enabling accurate predictions of performance metrics such as delay, jitter, and packet loss, even under highly dynamic conditions.

\subsubsection{Prior Work in Deep Learning-Based Network Modeling}
Early applications of Deep Learning (DL) to network modeling explored architectures such as Multilayer Perceptrons (MLPs) \textbf{CITATION} and Recurrent Neural Networks (RNNs) \textbf{CITATION}. These approaches leveraged the ability of neural networks to learn complex, non-linear relationships directly from data, bypassing the need for restrictive assumptions inherent in traditional methods like QT. While these models represented significant progress, their inherent limitations became apparent as networks grew in complexity and variability.

MLPs, as feedforward neural networks, have a fixed structure, requiring predefined input sizes. This rigidity makes them less suited for network modeling, where topologies, configurations, and traffic patterns vary dynamically. Table \ref{tab:traffic_model_mlp_rnn} illustrates this issue, showing MLPs perform reasonably well for simple traffic models like Poisson arrivals (MAPE = 12.3\%, $R^2$ = 0.801) but struggle with more complex patterns like Modulated Exponentials (MAPE = 57.1\%, $R^2$ = -1.679). These results highlight MLPs' difficulty in capturing the intricate dependencies and variability of real-world traffic.

RNNs, on the other hand, are designed to process sequential data, making them more adept at capturing temporal patterns in network traffic or packet flows. As shown in Table \ref{tab:traffic_model_mlp_rnn}, RNNs consistently outperform MLPs across all traffic models. For example, under On-Off traffic, RNNs achieve a lower MAPE (15.2\% vs. 30.4\%) and a higher $R^2$ (0.851 vs. 0.002). However, while RNNs excel at handling temporal dependencies, they are not inherently designed to represent the graph-structured nature of networks. Complex interdependencies between flows, links, and queues—such as traffic on overlapping routes or shared network resources—remain a challenge for RNNs.

\begin{table}[!htbp]
\caption{Delay prediction using an MLP and an RNN for different traffic models. The error is computed w.r.t. simulation results.}
\label{tab:traffic_model_mlp_rnn}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
     & \multicolumn{4}{c}{MLP}                 & \multicolumn{4}{c}{RNN}                \\
     \cmidrule(lr){2-5}
 \cmidrule(lr){6-9}
     & MAPE & MSE  & MAE  & R\textsuperscript{2} & MAPE & MSE  & MAE  & R\textsuperscript{2} \\
     \midrule
Poisson & 12.3\% & 0.103 & 0.122 & 0.801 & 10.0\% & 0.071 & 0.084 & 0.862 \\
Deterministic & 23.9\% & 0.309 & 0.160 & 0.044 & 13.1\% & 0.083 & 0.070 & 0.743 \\
On-Off & 30.4\% & 0.438 & 0.240 & 0.002 & 15.2\% & 0.065 & 0.082 & 0.851 \\
A. Exponentials & 84.5\% & 1.013 & 0.308 & -1.935 & 14.0\% & 0.070 & 0.072 & 0.7961 \\
M. Exponentials & 57.1\% & 1.058 & 0.363 & -1.679 & 57.8\% & 0.528 & 0.457 & -0.338 \\
Mixed & 41.2\% & 0.351 & 0.269 & 0.052 & 17.5\% & 0.036 & 0.080 & 0.900 \\
\bottomrule
\end{tabular}%
}
\end{table}

The limitations of these models are further emphasized when network configurations deviate from those seen during training. Table \ref{tab:mlp_rnn_routing_failures} compares the performance of MLPs and RNNs for the same routing configurations used in training, different routing configurations, and scenarios involving changes in topology (e.g., link failures). While both models perform reasonably well on the same routing configurations (MLP: MAPE = 12.3\%, $R^2$ = 0.801; RNN: MAPE = 10.0\%, $R^2$ = 0.862), their performance deteriorates significantly under new conditions. For instance, under different routing configurations, MLPs exhibit catastrophic errors (MAPE = 1150\%, $R^2$ = -40.0), and even RNNs, which are more robust, see a sharp decline in accuracy (MAPE = 30.5\%, $R^2$ = 0.197). Similarly, both models struggle with link failures, with RNNs performing marginally better (MAPE = 63.8\%, $R^2$ = 0.0417) than MLPs (MAPE = 125\%, $R^2$ = -0.191).

\begin{table}[!htbp]
\caption{Delay prediction using an MLP and an RNN for the same and different routing configurations w.r.t. those seen during training, and considering various link failures. The error is relative to simulation results.}
\label{tab:mlp_rnn_routing_failures}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
     & \multicolumn{4}{c}{MLP}                 & \multicolumn{4}{c}{RNN}                \\
     \cmidrule(lr){2-5}
 \cmidrule(lr){6-9}
     & MAPE & MSE  & MAE  & R\textsuperscript{2} & MAPE & MSE  & MAE  & R\textsuperscript{2} \\
     \midrule
Same Routing & 12.3\% & 0.103 & 0.122 & 0.801 & 10.0\% & 0.071 & 0.084 & 0.862 \\
Diff. Routing & 1150\% & 28.3 & 2.96 & -40.0 & 30.5\% & 0.553 & 0.282 & 0.197 \\
Diff. Topologies & 125\% & 3.69 & 1.03 & -0.191 & 63.8\% & 2.971 & 0.870 & 0.0417 \\
\bottomrule
\end{tabular}%
}
\end{table}

These results underline the limitations of MLPs and RNNs in scenarios involving dynamic network conditions. MLPs, due to their static structure, are inherently ill-suited for such variability. While RNNs can handle temporal sequences, their inability to natively model the graph structure of networks hampers their performance when faced with topological changes or failures. This highlights the need for models capable of directly representing and learning from the graph-based nature of networks to address these challenges effectively.


\subsubsection{Graph Neural Networks}
Graph Neural Networks (GNNs) have emerged as a transformative tool for network modeling. Unlike traditional neural networks, GNNs are designed to process graph-structured data, making them particularly suitable for representing computer networks where routers, links, and flows naturally form a graph. By dynamically adapting their architecture to the structure of the input graph, GNNs effectively capture the relationships between nodes and edges, enabling accurate predictions of performance metrics across diverse network scenarios.

\textbf{RouteNet} \textbf{CITE RouteNet-Models}, a family of GNN-based models, represents a significant advancement in this space. Unlike naive applications of GNNs directly to network graphs, RouteNet transforms the network's elements—such as flows, queues, and links—into specialized representations that reflect their roles and interactions within the network. Inspired by principles from Queuing Theory (QT), RouteNet incorporates flow-level information and models the interdependencies between flows and network components, such as shared queues and overlapping routes. This transformation enables RouteNet to predict key performance metrics like delay, jitter, and packet loss with remarkable accuracy, even for unseen scenarios or topologies.

To demonstrate why a vanilla application of GNNs to the network topology is insufficient, we evaluated four widely-used GNN architectures—GCN, GAT, GIN, and MPNN  \textbf{Add Citations}—against RouteNet. The models were tested across three scenarios:
1. Same routing configuration as the training data.
2. Different routing configurations.
3. Different topologies.

\begin{table}[!htbp]
\caption{Performance comparison of GNN architectures for delay prediction across different scenarios. Errors are relative to simulation results.}
\label{tab:gnn_comparison}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
     & \multicolumn{4}{c}{Same Routing}       & \multicolumn{4}{c}{Different Routing}  \\
     \cmidrule(lr){2-5}
     \cmidrule(lr){6-9}
     & MAPE & MSE  & MAE  & R\textsuperscript{2} & MAPE & MSE  & MAE  & R\textsuperscript{2} \\
     \midrule
GAT & 3.00\% & 0.051 & 0.041 & 0.945 & 15.00\% & 0.421 & 0.156 & 0.702 \\
GCN & 2.93\% & 0.047 & 0.040 & 0.948 & 16.69\% & 0.456 & 0.172 & 0.673 \\
GIN & 10.00\% & 0.203 & 0.098 & 0.814 & 16.10\% & 0.434 & 0.165 & 0.689 \\
MPNN & 2.98\% & 0.049 & 0.040 & 0.947 & 15.28\% & 0.437 & 0.161 & 0.695 \\
RouteNet & 1.66\% & 0.021 & 0.015 & 0.982 & 1.15\% & 0.012 & 0.009 & 0.995 \\
\midrule
     & \multicolumn{4}{c}{Different Topology} & \multicolumn{4}{c}{\textbf{Average Across Scenarios}} \\
     \cmidrule(lr){2-5}
     \cmidrule(lr){6-9}
     & MAPE & MSE  & MAE  & R\textsuperscript{2} & MAPE & MSE  & MAE  & R\textsuperscript{2} \\
     \midrule
GAT & 38.87\% & 1.923 & 0.589 & -0.412 & 18.29\% & 0.798 & 0.262 & 0.411 \\
GCN & 36.90\% & 1.843 & 0.572 & -0.389 & 18.17\% & 0.782 & 0.261 & 0.411 \\
GIN & 50.00\% & 2.435 & 0.718 & -0.921 & 25.37\% & 1.024 & 0.327 & 0.194 \\
MPNN & 37.80\% & 1.873 & 0.576 & -0.401 & 18.02\% & 0.786 & 0.259 & 0.417 \\
RouteNet & 2.17\% & 0.048 & 0.037 & 0.975 & 1.66\% & 0.027 & 0.020 & 0.984 \\
\bottomrule
\end{tabular}%
}
\end{table}

The results (shown in Table \ref{tab:gnn_comparison}) demonstrate that RouteNet significantly outperforms other GNN architectures across all scenarios. While models like GCN, GAT, and MPNN perform well under the same routing configurations as the training data, their performance deteriorates under different routing configurations or topologies. For instance, in the different topology scenario, MAPE for these models ranges from 36.9\% (GCN) to 50\% (GIN), whereas RouteNet achieves a much lower MAPE of 2.17\%. This illustrates the inability of general GNNs to generalize effectively to unseen scenarios without specialized transformations.

In contrast, RouteNet’s design captures the hierarchical relationships and dependencies within the network by explicitly modeling flows, queues, and links. This allows it to handle changes in routing configurations and topologies with remarkable accuracy (e.g., MAPE = 1.15\% for different routing configurations). These results highlight the need for domain-specific transformations in GNN-based approaches to unlock their full potential for network modeling.

\subsection{Real-World Scenarios}
Computer networks operate in highly dynamic environments where ensuring performance and reliability is paramount. RouteNet’s capabilities make it a powerful tool for addressing key challenges in real-world scenarios: Quality of Service (QoS), Generalization, and Real Nonstationary Traffic.

\subsubsection{Quality of Service and Scheduling Policies} QoS is a critical requirement in modern networks, ensuring that specific traffic flows meet performance guarantees such as low latency, high throughput, or prioritized delivery. QoS is often implemented using queue scheduling policies, including First In, First Out (FIFO), Weighted Fair Queuing (WFQ), Deficit Round Robin (DRR), and Strict Priority (SP), to allocate resources among flows based on their priorities.

\begin{table}[!htbp]
\caption{Benchmark of QT and RouteNet in the presence of Scheduling Policies for low, medium, and high traffic intensity.}
\label{tab:scheduling_delay}
\centering
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
     & \multicolumn{3}{c}{Delay} \\
     \cmidrule(lr){2-4}
     & Low & Medium  & High  \\
     \midrule
QT & 13.0\% & 17.3\% & 25.1\%  \\
RouteNet & 0.80\% & 2.60\% & 7.31\% \\
\bottomrule
\end{tabular}%
}
\end{table}

Table~\ref{tab:scheduling_delay} shows the results of evaluating RouteNet-F in scenarios with mixed scheduling policies, demonstrating its ability to accurately predict delay under different traffic intensities. RouteNet-F significantly outperforms the QT benchmark, highlighting its robustness and adaptability in modeling networks with QoS and diverse scheduling configurations.


\subsubsection{Generalization}
Generalization is a key challenge in data-driven network modeling. Unlike analytical methods like QT, which rely on assumptions, data-driven models require representative training datasets. These datasets must capture diverse network conditions, including varying congestion levels, routing configurations, and failure scenarios. However, production networks rarely experience extreme conditions such as severe congestion or link failures, making it challenging to generate such datasets in operational settings.

Controlled testbeds provide an effective alternative, allowing for the creation of synthetic datasets that replicate a wide range of network behaviors. RouteNet, trained on such diverse datasets, has demonstrated its ability to generalize effectively, accurately predicting performance even in scenarios involving previously unseen routing configurations or topologies. This generalization capability is essential for adapting to the dynamic nature of real-world networks.

To validate RouteNet’s ability to generalize to larger networks, we trained the model on small topologies with up to 10 nodes and evaluated it on networks of increasing size, ranging from 50 to 300 nodes. Table~\ref{tab:generalization_comparison} summarizes the results, showing that RouteNet consistently achieves low error rates, even for networks 30x larger than those seen during training. For example, the MAPE remains below 3.17\% for all topology sizes, with minimal differences from previous experiments. These results highlight RouteNet's robustness and adaptability, demonstrating its capacity to scale to significantly larger networks while maintaining high prediction accuracy.

\begin{table}[!htbp]
\caption{Generalization results of RouteNet evaluated on increasing topology sizes. The model was trained with topologies of up to 10 nodes.}
\label{tab:generalization_comparison}
\centering
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
Topology Size & MAPE & MSE & MAE & R\textsuperscript{2} \\
\midrule
50  & 0.76\% & 0.00004 & 0.001 & 0.996 \\
75  & 1.17\% & 0.00019 & 0.002 & 0.984 \\
100 & 1.89\% & 0.00016 & 0.003 & 0.980 \\
130 & 1.55\% & 0.00005 & 0.002 & 0.985 \\
170 & 2.43\% & 0.00008 & 0.002 & 0.978 \\
200 & 2.67\% & 0.00006 & 0.002 & 0.968 \\
240 & 2.58\% & 0.00007 & 0.002 & 0.979 \\
260 & 3.17\% & 0.00007 & 0.003 & 0.969 \\
280 & 3.16\% & 0.00003 & 0.002 & 0.979 \\
300 & 2.45\% & 0.00003 & 0.001 & 0.975 \\
\bottomrule
\end{tabular}%
}
\end{table}



\subsubsection{Non-Stationary Traffic}
Real-world networks often experience non-stationary traffic, where traffic patterns evolve due to changes in user behavior, network conditions, or external factors. Traditional RouteNet models are limited to predicting aggregate performance metrics over the duration of a flow, making them less suited for capturing temporal variations in traffic.

To address this limitation, a recent version of RouteNet, RouteNet-Gauss~\cite{güemespalau2025routenetgausshardwareenhancednetworkmodeling}, introduced a temporal component. By dividing network scenarios into fixed-size windows and processing each window independently, RouteNet-Gauss captures temporal dependencies and provides a detailed view of how flow performance metrics evolve. This advancement enables RouteNet to handle dynamic and non-stationary traffic patterns, a critical requirement for real-world network management.

\begin{table}[!htbp]
\caption{Windowed Performance Metrics per Dataset}
\label{tab:performance_metrics}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
{Dataset} & {Model} & {MAPE} & {MAE} & {R\textsuperscript{2}} \\
\midrule
\multirow{2}{*}{{Synthetic}} 
    & OMNeT++ & 53.68\% & 63.4857 & -4.3365 \\ 
    & RN-G    & 2.60\% & 3.1283  & 0.9413 \\ 
\midrule
\multirow{2}{*}{{Multi-Burst}} 
    & OMNeT++ & 56.12\% & 67.8069 & -4.5082 \\ 
    & RN-G    & 2.28\% & 2.8090  & 0.9211 \\ 
\midrule
\multirow{2}{*}{{RWPT}} 
    & OMNeT++ & 93.08\% & 126.0875 & -0.9909 \\ 
    & RN-G    & 14.75\% & 47.2170  & 0.0553 \\ 
\bottomrule
\end{tabular}%
}
\end{table}

Table~\ref{tab:performance_metrics} presents the performance of RouteNet-Gauss (RN-G) compared to the OMNeT++ simulator across three datasets that reflect varying traffic dynamics: Synthetic traffic with high-frequency bursts, Multi-Burst traffic, and Real-World Packet Traces (RWPT). While machine learning models like RouteNet-Gauss demonstrate strong performance across these datasets, OMNeT++ exhibits significantly higher error rates, particularly for more complex traffic patterns such as RWPT. This discrepancy highlights a common limitation of traditional network simulators like OMNeT++, which are designed to operate under idealized conditions with controlled and well-defined traffic assumptions. However, real-world network environments often deviate from these idealizations due to dynamic and non-stationary factors such as bursty traffic, unexpected congestion, and varying flow priorities. As a result, simulators like OMNeT++ struggle to maintain accuracy when faced with the variability and complexity of real-world conditions, underscoring the need for adaptive, data-driven approaches like RouteNet-Gauss.




==> sections/appendices/applicability.tex <==
TODO: introductory paragraph

\paragraph{Scheduling Policies.} In order to ensure that specific traffic flows meet performance guarantees such as low latency, high throughput, or prioritized delivery, RouteNet is compatible with different queue scheduling policies, enabling to allocate resources among flows based on their priorities. %Some implemented policies are First In, First Out (FIFO), Weighted Fair Queuing (WFQ), Deficit Round Robin (DRR), and Strict Priority (SP). 
Table~\ref{tab:scheduling_delay} shows the results of evaluating RouteNet in scenarios with mixed scheduling policies, demonstrating its ability to accurately predict delay under different traffic intensities and diverse scheduling configurations. %RouteNet-F significantly outperforms the QT benchmark, highlighting its robustness and adaptability in modeling networks with QoS and diverse scheduling configurations.

\begin{table}[!t]
\caption{Benchmark of QT and RouteNet in the presence of Scheduling Policies for low, medium, and high traffic intensity.}
\label{tab:scheduling_delay}
\centering
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
     & \multicolumn{3}{c}{Traffic Intensity} \\
     \cmidrule(lr){2-4}
     & Low & Medium  & High  \\
     \midrule
QT & 13.0\% & 17.3\% & 25.1\%  \\
RouteNet & 0.80\% & 2.60\% & 7.31\% \\
\bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[!t]
\caption{Generalization results of RouteNet evaluated on increasing topology sizes. The model was trained with topologies of up to 10 nodes.}
\label{tab:generalization_comparison}
\centering
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{ccccc}
\toprule
Topology Size & MAPE & MSE & MAE  \\
\midrule
50  & 0.76\% & 0.00004 & 0.001  \\
% 75  & 1.17\% & 0.00019 & 0.002 & 0.984 \\
100 & 1.89\% & 0.00016 & 0.003  \\
% 130 & 1.55\% & 0.00005 & 0.002 & 0.985 \\
% 170 & 2.43\% & 0.00008 & 0.002 & 0.978 \\
200 & 2.67\% & 0.00006 & 0.002  \\
% 240 & 2.58\% & 0.00007 & 0.002 & 0.979 \\
% 260 & 3.17\% & 0.00007 & 0.003 & 0.969 \\
% 280 & 3.16\% & 0.00003 & 0.002 & 0.979 \\
300 & 2.45\% & 0.00003 & 0.001  \\
\bottomrule
\end{tabular}%
}
\end{table}

\paragraph{Scalability.}
Scalability is a key challenge in data-driven network modeling. Unlike analytical methods like QT, which rely on assumptions, data-driven models require training datasets capturing diverse network conditions. However, production networks rarely experience extreme conditions such as severe congestion or link failures, making it challenging to generate such datasets in operational settings. 
Controlled testbeds provide an effective alternative, allowing for the creation of synthetic datasets that replicate a wide range of network behaviors. However, network testbeds are usually much smaller than real networks. 
%RouteNet, trained on such diverse datasets, has demonstrated its ability to generalize effectively, accurately predicting performance even in scenarios involving previously unseen routing configurations or topologies. This generalization capability is essential for adapting to the dynamic nature of real-world networks. 
To validate RouteNet’s ability to scale to larger networks, the model was trained on small topologies with up to 10 nodes and then evaluated on networks of increasing size, ranging from 50 to 300 nodes. Table~\ref{tab:generalization_comparison} summarizes the results, showing that RouteNet consistently achieves low error rates, even for networks 30x larger than those seen during training. 
%For example, the MAPE remains below 3.17\% for all topology sizes, with minimal differences from previous experiments. These results highlight RouteNet's robustness and adaptability, demonstrating its capacity to scale to significantly larger networks while maintaining high prediction accuracy.

\begin{table}[!t]
\caption{Windowed Performance Metrics per Dataset}
\label{tab:performance_metrics}
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
{Dataset} & {Model} & {MAPE} & {MAE}  \\
\midrule
\multirow{2}{*}{{Synthetic}} 
    & OMNeT++ & 53.68\% & 63.4857  \\ 
    & RN-G    & 2.60\% & 3.1283  \\ 
\midrule
\multirow{2}{*}{{Multi-Burst}} 
    & OMNeT++ & 56.12\% & 67.8069  \\ 
    & RN-G    & 2.28\% & 2.8090   \\ 
\midrule
\multirow{2}{*}{{RWPT}} 
    & OMNeT++ & 93.08\% & 126.0875  \\ 
    & RN-G    & 14.75\% & 47.2170   \\ 
\bottomrule
\end{tabular}%
}
\end{table}

\paragraph{Non-Stationary Traffic}
Real-world networks often experience non-stationary traffic, where traffic patterns evolve due to changes in user behavior, network conditions, or external factors. Traditional RouteNet models are limited to predicting aggregate performance metrics over the duration of a flow, making them less suited for capturing temporal variations in traffic. 
To address this limitation, the latest RouteNet version %a recent version of RouteNet, RouteNet-Gauss~\cite{güemespalau2025routenetgausshardwareenhancednetworkmodeling}, 
introduces a temporal component. By dividing network scenarios into fixed-size windows and processing each window independently, it captures temporal dependencies and provides a detailed view of how flow performance metrics evolve. This advancement enables RouteNet to handle dynamic and non-stationary traffic patterns, a critical requirement for real-world network management. 
Table~\ref{tab:performance_metrics} presents the performance of RouteNet compared to the OMNeT++ simulator across three datasets that reflect varying traffic dynamics: Synthetic traffic with high-frequency bursts, Multi-Burst traffic, and Real-World Packet Traces (RWPT). 
% [SUMMARIZE RESULTS IN A HEADLINE]
Overall, RouteNet proved to be more faithful while replicating the packet's behavior than the OMNeT++ simulator, both in synthetic and real traffic distributions, decreasing the MAPE by 84\% in the latter.
%While machine learning models like RouteNet-Gauss demonstrate strong performance across these datasets, OMNeT++ exhibits significantly higher error rates, particularly for more complex traffic patterns such as RWPT. This discrepancy highlights a common limitation of traditional network simulators like OMNeT++, which are designed to operate under idealized conditions with controlled and well-defined traffic assumptions. However, real-world network environments often deviate from these idealizations due to dynamic and non-stationary factors such as bursty traffic, unexpected congestion, and varying flow priorities. As a result, simulators like OMNeT++ struggle to maintain accuracy when faced with the variability and complexity of real-world conditions, underscoring the need for adaptive, data-driven approaches like RouteNet-Gauss.


% \paragraph{Deployment.} [MAYBE MENTION FEASIBILITY OF DEPLOYMENT? HIGHLIGHTING ALL PREVIOUS FEATURES]

==> sections/networking.tex <==
Network modeling is a cornerstone of computer network research, design, and operations. %It enables the simulation and analysis of network behavior, which is crucial for tasks such as protocol development, performance evaluation, and network optimization. 
By abstracting the network’s physical and logical components, it enables the simulation and analysis of network behavior, helping predict performance metrics (such as delay and jitter) under different configurations and workloads in a controlled environment. 
%models help researchers and engineers predict performance metrics --such as delay and jitter-- under different configurations and workloads. %Over the years, network modeling has been applied in diverse areas, including traffic engineering, capacity planning, and Quality of Service (QoS) assurance.
This section reviews the most relevant methodologies currently leveraged in this field. 

\vspace{5pt}
\noindent\textbf{Experimental Results.} To help contextualize each of the considered methods, this section is also supported by a selected set of experimental scenarios extracted from different RouteNet publications. However, we have re-run RouteNet and the ML baselines in each of the considered configurations to obtain the result values shown in our tables and figures. Details about training and evaluation datasets can be found in Appendix~\ref{app:network_data}, while further experimental setup specifications can be found in Appendix~\ref{app:routenet_experiments}. 

\paragraph{Packet-Level Simulators.}
Packet-level simulators, such as ns-3 \cite{riley2010ns} and OMNeT++ \cite{varga2001discrete}, provide detailed modeling by simulating network behavior at the granularity of individual packets. These tools offer high accuracy and flexibility, allowing researchers to include various features such as routing algorithms, scheduling policies, and traffic patterns. However, their main limitation is computational cost. Simulation time typically grows linearly with the number of packets processed, making these tools impractical for large-scale networks or real-time applications. %For instance, simulating a high-speed link (e.g., 10 Gbps) over a realistic traffic volume can take hours or even days. 
%[ADD HERE DONS, DQN, MIMICNET]
Efforts to address this limitation have focused on improving efficiency through parallelization and machine learning \citep{gao2023dons,yang2022deepqueuenet,zhang2021mimicnet}, but --as illustrated in Figure \ref{fig:simulation_cost}-- they remain several orders of magnitude more computationally expensive than other alternatives.
%. \textbf{DONS} (Distributed Omnet++ Simulation) \cite{gao2023dons} partitions networks and processes them in parallel, achieving up to 65x speedup over traditional sequential simulators. \textbf{Deep Queue Net (DQN)} \cite{yang2022deepqueuenet} leverages transformers and multi-GPU acceleration to model packet dynamics more efficiently. \textbf{MimicNet} \cite{zhang2021mimicnet} combines machine learning with packet-level simulations to reduce computational overhead, but its applicability is limited to specific topologies. While these approaches improve scalability, packet-level simulations remain computationally expensive, especially for large-scale or time-sensitive scenarios.


% Efforts to address this limitation have focused on parallelizing the simulation process to improve efficiency. For instance, DONS (Distributed Omnet++ Simulation) \textbf{CITE DONS} achieves up to 65x speedup over traditional sequential simulators by partitioning networks and processing them in parallel. Similarly, approaches like Deep Queue Net (DQN) leverage transformers and multi-GPU configurations to significantly accelerate computational times.

% Figure \ref{fig:simulation_cost} illustrates simulation times for several link speeds commonly found in modern networks. The results show that even with advancements like DONS and DQN, packet-level simulators remain computationally expensive, particularly for high-speed links. 



\paragraph{Queuing Theory.}
Queuing Theory (QT) has been a basis of network modeling for decades and remains one of the most widely used analytical techniques in the field. Its importance stems from its ability to provide a mathematical framework to model networks as a set of interconnected queues. Each queue represents a network component, such as a router or switch, handling data packets. %QT’s dominance in network modeling lies in its simplicity and efficiency. 
Unlike packet-level simulators, which require extensive computation to simulate individual packets, QT uses mathematical models to derive performance metrics directly. For example, it assumes that traffic follows a Poisson arrival process and that queues behave according to Markovian principles. These assumptions make QT computationally fast and well-suited for large-scale networks or scenarios where quick predictions are required. 
However, the strength of QT is also its main limitation: the simplifying assumptions that make it efficient often fail to capture the complexities of real-world network traffic. %Studies have shown that modern network traffic exhibits properties like strong autocorrelation and heavy-tailed distributions [CITATIONS], which deviate significantly from the idealized Poisson and Markovian models. 
This is evident in the results shown in Table \ref{tab:traffic_models}, where QT's performance in delay prediction varies significantly across different traffic models.

\begin{figure}[!t] \centering \includegraphics[width=\columnwidth]{./figures/motivation_cost_v3.pdf} \caption{Inference times for 1 second of a real 14-node topology depending on the amount of traffic found in the network. Results demonstrate the significant computational cost of packet-level simulations, even with advanced techniques.} \label{fig:simulation_cost} 
\end{figure}

\paragraph{Early Data-driven Approaches.}
Early applications of Deep Learning (DL) to network modeling explored architectures such as Multilayer Perceptrons (MLPs)~\cite{sadeghzadeh2008mlp, mestres2018understanding, wang2017machine} and Recurrent Neural Networks (RNNs)~\cite{belhaj2009modeling, mohammed2019machine, naseer2018enhanced}. These approaches leveraged the ability of neural networks to learn complex, non-linear relationships directly from data, bypassing the need for restrictive assumptions inherent in traditional methods like QT. However, while these models represented significant progress, Table \ref{tab:traffic_models} shows their inherent limitations. On the one hand, MLPs have a fixed structure, requiring predefined input sizes. This rigidity makes them less suited for network modeling, where topologies, configurations, and traffic patterns vary dynamically. RNNs, on the other hand, are designed to process sequential data, making them more adept at capturing temporal patterns in network traffic or packet flows. However, they are not inherently designed to represent the graph-structured inter-dependencies between flows, links, and queues --such as traffic on overlapping routes or shared network resources. 

\paragraph{Pairwise Relationships: The Emergence of GNNs.} The limitations of MLP and RNN models are further emphasized when network configurations deviate from those seen during training. As underlined in Table \ref{tab:different_routing_topologies}, their performance deteriorates significantly with different routing configurations and changes in topology (e.g., link failures). In this context, GNNs emerged as a transformative tool for network modeling. By dynamically adapting their architecture to the structure of the input network graph topology, GNNs can effectively capture the relationships between different routers and links, thus enabling more accurate predictions of performance metrics across diverse network scenarios. Table \ref{tab:different_routing_topologies} shows how different well-known GNN implementations (GCN~\citep{kipf2017semi}, GAT~\citep{velickovic2017graph}, GIN~\citep{xu2018how}, MPNN~\cite{gilmer2017neural}) clearly outperform previous ML architectures. However, despite the overall improvement, we can observe that vanilla GNN architectures still struggle to keep comparable performance when considering routing and topologies not seen in training.

\paragraph{Higher-Order Relationships: RouteNet.} The RouteNet family of models~\cite{rusek2020routenet, ferriol2022routenet, ferriol2023routenet, guemes2025routenet} represents a significant advance in this regard. Unlike vanilla applications of GNNs, RouteNet transforms the network's elements --such as flows, queues, and links-- into specialized representations that reflect their roles and interactions within the network. Inspired by principles from QT, RouteNet incorporates flow-level information and models the interdependencies between flows and network components (such as shared queues and overlapping routes). This transformation enables RouteNet to predict key performance metrics like delay, jitter, and packet loss with remarkable accuracy, even for unseen scenarios or topologies, while keeping an execution time comparable to that of QT methodologies --see Table \ref{tab:different_routing_topologies} and Figure \ref{fig:simulation_cost}). Additionally, the subsequent versions of RouteNet have successfully overcome relevant real-world deployment challenges --e.g., by supporting several scheduling policies, scaling to networks way larger than those seen in training, or handling real-world non-stationary traffic. We further expand on these capabilities in Appendix \ref{app:deployment}, including the corresponding experimental results.


% \paragraph{The Applicability of RouteNet.}  
% RouteNet has demonstrated its versatility across different network modeling challenges. First, it supports various \textbf{scheduling policies}, making it capable of understanding \textbf{Quality of Service (QoS)} configurations by accurately modeling how different queuing mechanisms impact network performance. Second, it exhibits strong \textbf{scalability}, maintaining low error rates even when evaluated on networks up to 30 times larger than those seen during training. This generalization capability is crucial for training on small, controlled testbeds while ensuring reliable deployment in large-scale production networks. Additionally, RouteNet effectively handles \textbf{non-stationary traffic} by incorporating a temporal component, enabling it to model dynamic network conditions more accurately than classical simulation tools. We refer the reader to Appendix \ref{app:routenet_evolution} for a more detailed explanation of these capabilities.




\input{tables/different_routings_topologies}


% The results (shown in Table \ref{tab:gnn_comparison}) demonstrate that RouteNet significantly outperforms other GNN architectures across all scenarios. While models like GCN, GAT, and MPNN perform well under the same routing configurations as the training data, their performance deteriorates under different routing configurations or topologies. For instance, in the different topology scenario, MAPE for these models ranges from 36.9\% (GCN) to 50\% (GIN), whereas RouteNet achieves a much lower MAPE of 2.17\%. This illustrates the inability of general GNNs to generalize effectively to unseen scenarios without specialized transformations.

==> sections/results.tex <==
\begin{table}[ht]
    \centering
    \caption{Performance Metrics by Dataset}
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Dataset} & \textbf{Model} & \textbf{MAPE} & \textbf{MSE} & \textbf{MAE} & \textbf{R2} \\
        \midrule
        \multirow{4}{*}{\textbf{NSFNET}} 
            & MLP      & 0.4611 & 4.2370 & 0.7794 & -0.1586 \\
            & RNN      & 0.6670 & 4.3660 & 0.8471 & -0.1939 \\
            & MPNN     & 0.2258 & 3.7314 & 0.6431 & -0.0203 \\
            & RN-F     & 0.0333 & 0.0773 & 0.0637 & 0.9789 \\
        \midrule
        \multirow{4}{*}{\textbf{GEANT}} 
            & MLP      & 0.3588 & 1.1145 & 0.3031 & -0.0392 \\
            & RNN      & 0.5820 & 1.1727 & 0.3367 & -0.0934 \\
            & MPNN     & 0.2067 & 1.0343 & 0.2694 & 0.0357 \\
            & RN-F     & 0.0398 & 0.0281 & 0.0346 & 0.9738 \\
        \midrule
        \multirow{4}{*}{\textbf{GBN}} 
            & MLP      & 0.8747 & 3.0930 & 0.5374 & -0.0788 \\
            & RNN      & 0.5340 & 3.1246 & 0.5233 & -0.0898 \\
            & MPNN     & 0.2196 & 2.8427 & 0.4380 & 0.0085 \\
            & RN-F     & 0.0347 & 0.0678 & 0.0461 & 0.9764 \\
        \midrule
        \multirow{4}{*}{\textbf{Topology ZOO}} 
            & MLP      & 0.8529 & 16.8645 & 0.3365 & -0.1743 \\
            & RNN      & 0.6436 & 14.4481 & 0.3221 & -0.0061 \\
            & MPNN     & 0.7329 & 10.5993 & 0.2898 & 0.2619 \\
            & RN-F     & 0.0389 & 0.4762 & 0.0259 & 0.9668 \\
        \bottomrule
    \end{tabular}
    \label{tab:performance_metrics}
\end{table}

==> sections/temporal_domain.tex <==
% Real traffic is non-stationary, RouteNet by itself struggles with it
One of the limitations of the methodology of the discussed RouteNet models are its inability to deal with non-stationary traffic. This is as a result of RouteNet only being able to predict aggregate performance metrics for the entirety of the flow's duration.

% RouteNet-G fixes this by considering the temporal domain through fixed-size windows. Windows are processed independently
However, this was addressed by the authors when building RouteNet-Gauss~\cite{güemespalau2025routenetgausshardwareenhancednetworkmodeling} by including in the model a temporal component. Doing so grants the model the ability to describe the flow's performance metrics as they evolve over its duration. More specifically, RouteNet-Gauss divides the network scenario into fixed-sized windows.

% Initial features can be encoded in one of two ways: flows and links states can be encoded with time-dependent feature, whose value will change at each window. Nodes, whose features aren't, are encoded once and then the representation is shared across windows
Each window is processed independently, and the temporal information and temporal dependencies are introduced while encoding the internal representations of each of the network element. On the one hand flows and links can be encoded directly and independently using observable, time-dependent features. These include ones such as the current flow bandwidth or link load.

%Nodes, whose features are either time-independent, or unobservable or latent, instead only get encoded once at the first window. For following windows, its initial encoding will be the output for the same element, in the previous window, after the final DirTNN layer.
On the other hand, the queues on routers are harder to encode. This is because these can only be described through time-independent features (e.g. router's specifications) or ones that are not possible to measure in real time (e.g. buffer usage). Instead RouteNet-Gauss follows the following approach: for the initial window, $\prescript{(0)}{}{h_{q}^{0}}$, queues are encoded using the static features. Then, for consequent windows $w$, queues re-use the final encoding obtained after all the GNN layers (or DirTNN layers when applied to TopoRouteNet) in the previous window: $\prescript{(w)}{}{h_{q}^{0}} \leftarrow \prescript{(w-1)}{}{h_{q}^{L}}$.

% Testbed network used to evaluate
This model was then trained and evaluated with real traffic generated from a testbed network. The testbed included 8 high-capacity routers, with software defined routings so it can replicate the structure of any topology of that size. Two traffic generator servers inject traffic into the network, either following a synthetic traffic distribution or replicating the measurements stored in provided packet-capture files. The testbed capacity was provisioned to have a similar capacity to modern network, with link capacities no smaller than 1 Gbps.

\begin{table}[ht]
    \centering
    \caption{Windowed Performance Metrics per dataset}
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Dataset} & \textbf{Metric} & \textbf{Model} & \textbf{MAPE} & \textbf{MAE} & \textbf{R2} \\
        \midrule
        \multirow{4}{*}{\textbf{TREX-S}}
            & \multirow{2}{*}{\textbf{Delay}} &  OMNeT++ & 0.5368 & 63.4857 & -4.3365 \\ 
            & & RN-G & 0.0260 & 3.1283 & 0.9413 \\ \cline{2-6} 
            & \multirow{2}{*}{\textbf{Jitter}} &  OMNeT++ & 0.2500 & 2.1222 & -0.5845 \\ 
            & & RN-G & 0.0945 & 0.7917 & 0.7575 \\ \midrule
        \multirow{4}{*}{\textbf{TREX-MB}}
            & \multirow{2}{*}{\textbf{Delay}} &  OMNeT++ & 0.5612 & 67.8069 & -4.5082 \\ 
            & & RN-G & 0.0228 & 2.8090 & 0.9211 \\ \cline{2-6} 
            & \multirow{2}{*}{\textbf{Jitter}} &  OMNeT++ & 0.3743 & 3.2444 & -1.9798 \\ 
            & & RN-G & 0.1071 & 0.9668 & 0.5294 \\ \midrule 
        \multirow{4}{*}{\textbf{RWPT}}
            & \multirow{2}{*}{\textbf{Delay}} &  OMNeT++ & 0.9308 & 126.0875 & -0.9909 \\ 
            & & RN-G & 0.1475 & 47.2170 & 0.0553 \\ \cline{2-6} 
            & \multirow{2}{*}{\textbf{Jitter}} &  OMNeT++ & 0.4644 & 6.5898 & -0.9594 \\ 
            & & RN-G & 0.1445 & 2.3351 & 0.5900 \\
        \bottomrule
    \end{tabular}
    \label{tab:performance_metrics}
\end{table}

==> sections/toporoutenet.tex <==
%We need a visual representation of the network, and how it translates to the model.

Computer networks can be straightforwardly modeled as a graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$, with the set of nodes $\mathcal{V}$ representing hardware devices (like routers or switches), and the set of edges $\mathcal{E}$ depicting the physical or wireless links that connect them. Narrowing down the scope to the network modeling scenarios considered by the RouteNet family of methods, in this paper we will focus on wired ISP-based networks.

However, RouteNet success can actually be accounted for going beyond this direct one-to-one correspondence network-graph. One key aspect of their design is to explicitly incorporate traffic flows into the model architecture. Notably, these flows induce higher-order substructures within the graph, reflecting traffic paths occurring in the network between source-destination pairs of nodes.

Another relevant feature --introduced in the most recent models-- is that the considered set of nodes do not represent the network routers, but rather the collection of all router queues. More specifically, routers internally implement different queues, being in most cases a valid assumption to consider one for each of the outgoing links. Such decoupling of routers into independent queue-based nodes has enabled a finer-grained and more accurate modeling of the network dynamics, as supported by empirical evidence.

So, overall, RouteNet ends up building a computational model that both extends and stretches the original graph-based network topology. Although originally devised as a heterogeneous GNN-based solution with a sophisticated multi-step message-passing procedure, we show as follows that it can be naturally formulated as a DirTNN.

\begin{proposition} \label{prop:combinatorial_representation}
    RouteNet's internal representation of a computer network can be fully described as a combinatorial complex $\mathcal{C}$ such that
    \begin{itemize}
        \item the set of nodes $\mathcal{V}$ represent queues on routers;
        \item 1-cells $\mathcal{E}$ represent the wired links of the computer network;
        \item 2-cells $\mathcal{F}$ represent the set of flows traversing the network. 
    \end{itemize}
\end{proposition}

\begin{proposition} \label{prop:toporoutenet}
    RouteNet's internal modeling of a computer network can be formulated as a DirTNN. In particular, the hidden states' update equations for a flow $f\in \mathcal{F}$, a queue $q\in \mathcal{V}$, and a link $e\in \mathcal{E}$ are, respectively,
    \begin{equation} \label{eq:flow_update}
        h_{f}^{t+1} = \bigoplus_{l \in \Delta_f^1} h_{f,l}^{t+1},
    \end{equation}
    \begin{equation} \label{eq:queue_update}
        h_{q}^{t+1} = \Phi \left(h_q^t, \bigoplus_{f \in \mathcal{N}_{I, \uparrow}^{2}(q)} h_{f,q}^{t+1} \right),
    \end{equation}
    \begin{equation} \label{eq:link_update}
        h_{l}^{t+1} = \Theta \left(h_l^t, \bigoplus_{q \in \Delta_l^0} h_{q}^{t+1} \right),
    \end{equation}
    where 
    \begin{equation} \label{eq:face_dependent_update}
        h_{f,l}^{t+1} = h_{f,q}^{t+1} =\psi \left( h_f^t , \bigoplus_{\substack{ l' \in \Delta_f^1[\leq l] \\ \ q' = \Delta_{l'}^0[0]}} \phi (h_{q'}^t,h_{l'}^t) \right)
    \end{equation}
    are the face-dependent flow representations.
\end{proposition}

Proofs can be found in Appendices \ref{app:proof_combinatorial_representation} and \ref{app:proof_toporoutenet}, respectively. Notably, the aggregators $\bigoplus$ of Eqs. \eqref{eq:flow_update}, \eqref{eq:queue_update}, and \eqref{eq:face_dependent_update} are implemented as recurrent neural network --Gated Recurring Units (GRUs) [CITATION]-- in order to exploit the order induced by flows over queues and links. Additional technical details on RouteNet's architecture can be found in Appendix \ref{app:routenet_technical_details}.





==> tables/different_routings_topologies.tex <==
\begin{table}[!t]
\caption{Performance comparison of different ML architectures for the same and different routing configurations and topologies w.r.t. those seen during training.}
\label{tab:different_routing_topologies}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccccccc}
\toprule
     & \multicolumn{3}{c}{Same Routing}       & \multicolumn{3}{c}{Different Routing} & \multicolumn{3}{c}{Different Topologies}  \\
     \cmidrule(lr){2-4}
     \cmidrule(lr){5-7}
     \cmidrule(lr){8-10}
     & MAPE & MSE  & MAE  & MAPE & MSE  & MAE & MAPE & MSE  & MAE   \\
     \midrule
MLP & 12.3\% & 0.103 & 0.122 & 1150\% & 28.3 & 2.96 & 125\% & 3.69 & 1.03 \\
RNN & 10.0\% & 0.071 & 0.084 & 30.5\% & 0.553 & 0.282 & 63.8\% & 2.971 & 0.870 \\ 
\midrule
GAT & 3.00\% & 0.051 & 0.041 & 15.00\% & 0.421 & 0.156 & 38.87\% & 1.923 & 0.589  \\
GCN & 2.93\% & 0.047 & 0.040 & 16.69\% & 0.456 & 0.172 & 36.90\% & 1.843 & 0.572  \\
GIN & 10.00\% & 0.203 & 0.098 & 16.10\% & 0.434 & 0.165 & 50.00\% & 2.435 & 0.718  \\
MPNN & 2.98\% & 0.049 & 0.040 & 15.28\% & 0.437 & 0.161 & 37.80\% & 1.873 & 0.576  \\
\midrule
No-Order & 2.6\% & 3.1283 & 47.4655 & 2.28\% & 2.81 & 71.6149 & 14.75\% & 47.22 & 95.4291  \\
No-Order-MP & 2.6\% & 3.1283 & 47.4655 & 2.28\% & 2.81 & 71.6149 & 14.75\% & 47.22 & 95.4291  \\
\midrule
RouteNet & \textbf{1.66\%} & \textbf{0.001} & \textbf{0.015} & \textbf{1.15\%} & \textbf{0.012} & \textbf{0.009} &  \textbf{2.17\%} & \textbf{0.048} & \textbf{0.037}  \\
\bottomrule
\end{tabular}%
}
\end{table}


%%%%%%%%% OLD TABLES %%%%%%%%%%%

% \begin{table}[!htbp]
% \caption{Delay prediction using an MLP and an RNN for the same and different routing configurations w.r.t. those seen during training, and considering various link failures. The error is relative to simulation results.}
% \label{tab:mlp_rnn_routing_failures}
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ccccccccc}
% \toprule
%      & \multicolumn{4}{c}{MLP}                 & \multicolumn{4}{c}{RNN}                \\
%      \cmidrule(lr){2-5}
%  \cmidrule(lr){6-9}
%      & MAPE & MSE  & MAE  & R\textsuperscript{2} & MAPE & MSE  & MAE  & R\textsuperscript{2} \\
%      \midrule
% Same Routing & 12.3\% & 0.103 & 0.122 & 0.801 & 10.0\% & 0.071 & 0.084 & 0.862 \\
% Diff. Routing & 1150\% & 28.3 & 2.96 & -40.0 & 30.5\% & 0.553 & 0.282 & 0.197 \\
% Diff. Topologies & 125\% & 3.69 & 1.03 & -0.191 & 63.8\% & 2.971 & 0.870 & 0.0417 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}


% \begin{table}[!htbp]
% \caption{Performance comparison of GNN architectures for delay prediction across different scenarios. Errors are relative to simulation results.}
% \label{tab:gnn_comparison}
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ccccccccc}
% \toprule
%      & \multicolumn{4}{c}{Same Routing}       & \multicolumn{4}{c}{Different Routing}  \\
%      \cmidrule(lr){2-5}
%      \cmidrule(lr){6-9}
%      & MAPE & MSE  & MAE  & R\textsuperscript{2} & MAPE & MSE  & MAE  & R\textsuperscript{2} \\
%      \midrule
% GAT & 3.00\% & 0.051 & 0.041 & 0.945 & 15.00\% & 0.421 & 0.156 & 0.702 \\
% GCN & 2.93\% & 0.047 & 0.040 & 0.948 & 16.69\% & 0.456 & 0.172 & 0.673 \\
% GIN & 10.00\% & 0.203 & 0.098 & 0.814 & 16.10\% & 0.434 & 0.165 & 0.689 \\
% MPNN & 2.98\% & 0.049 & 0.040 & 0.947 & 15.28\% & 0.437 & 0.161 & 0.695 \\
% RouteNet & 1.66\% & 0.021 & 0.015 & 0.982 & 1.15\% & 0.012 & 0.009 & 0.995 \\
% \midrule
%      & \multicolumn{4}{c}{Different Topology} & \multicolumn{4}{c}{\textbf{Average Across Scenarios}} \\
%      \cmidrule(lr){2-5}
%      \cmidrule(lr){6-9}
%      & MAPE & MSE  & MAE  & R\textsuperscript{2} & MAPE & MSE  & MAE  & R\textsuperscript{2} \\
%      \midrule
% GAT & 38.87\% & 1.923 & 0.589 & -0.412 & 18.29\% & 0.798 & 0.262 & 0.411 \\
% GCN & 36.90\% & 1.843 & 0.572 & -0.389 & 18.17\% & 0.782 & 0.261 & 0.411 \\
% GIN & 50.00\% & 2.435 & 0.718 & -0.921 & 25.37\% & 1.024 & 0.327 & 0.194 \\
% MPNN & 37.80\% & 1.873 & 0.576 & -0.401 & 18.02\% & 0.786 & 0.259 & 0.417 \\
% RouteNet & 2.17\% & 0.048 & 0.037 & 0.975 & 1.66\% & 0.027 & 0.020 & 0.984 \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}

==> tables/testbed.tex <==
\begin{table}[!t]
\caption{Performance comparison of different ML architectures for multiple routing configurations and topologies in a real testbed.}
\label{tab:real_testbed}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccccccc}
\toprule
     & \multicolumn{3}{c}{Synthetic}       & \multicolumn{3}{c}{Multi-Burst} & \multicolumn{3}{c}{MAWI}  \\
     \cmidrule(lr){2-4}
     \cmidrule(lr){5-7}
     \cmidrule(lr){8-10}
     & MAPE & MSE  & MAE  & MAPE & MSE  & MAE & MAPE & MSE  & MAE   \\
     \midrule
OMNeT++ & 53.68\% & 4313.42 & 63.48 & 56.12\% & 4997.01 & 67.80 & 93.08\% & \(1.40\!\times\!10^5\) & 126.087 \\
\midrule
MLP & \(3.58\!\times\!10^{13}\)\% & \(4.95\!\times\!10^5\) & 418.60 & \(4.91\!\times\!10^{13}\)\% & \(1.45\!\times\!10^6\) & 649.36 & \(4.89\!\times\!10^{13}\)\% & \(4.57\!\times\!10^5\) & 261.69 \\
RNN & 19.28\% & 1013.86 & 24.65 & \(2.79\!\times\!10^8\)\% & \(3.00\!\times\!10^{17}\) & \(2.54\!\times\!10^8\) & 29.98\% & \(1.21\!\times\!10^4\) & 49.52 \\
\midrule
GAT & 23.52\% & \(2.30\!\times\!10^4\) & 28.15 & 29.02\% & \(1.48\!\times\!10^4\) & 32.29 & 29.96\% & \(1.17\!\times\!10^4\) & 48.12 \\
GCN & 19.48\% & 847.08 & 23.29 & 19.08\% & 909.54 & 23.62 & 29.92\% & \(1.20\!\times\!10^4\) & 49.15 \\
GIN & 19.78\% & 1148.26 & 25.98 & 531.77\% & \(7.35\!\times\!10^5\) & 544.56 & 30.04\% & \(1.16\!\times\!10^4\) & 47.85 \\
MPNN & 19.48\% & 847.44 & 23.29 & 406.16\% & \(1.62\!\times\!10^6\) & 434.76 & 29.90\% & \(1.19\!\times\!10^4\) & 48.71 \\
\midrule
No-Order & 19.48\% & 847.44 & 23.29 & 406.16\% & \(1.62\!\times\!10^6\) & 434.76 & 29.90\% & \(1.19\!\times\!10^4\) & 48.71 \\
No-Order-MP & 19.48\% & 847.44 & 23.29 & 406.16\% & \(1.62\!\times\!10^6\) & 434.76 & 29.90\% & \(1.19\!\times\!10^4\) & 48.71 \\
\midrule
RouteNet & 2.6\% & 3.1283 & 47.4655 & 2.28\% & 2.81 & 71.6149 & 14.75\% & 47.22 & 95.4291  \\
\bottomrule
\end{tabular}%
}
\end{table}

